On the stability, correctness and plausibility of visual explanation methods based on feature importance

In the field of Explainable AI, multiples evaluation metrics have been proposed in order to assess the quality of explanation methods w.r.t. a set of desired properties. In this work, we study the articulation between the stability, correctness and plausibility of explanations based on feature importance for image classifiers. We show that the existing metrics for evaluating these properties do not always agree, raising the issue of what constitutes a good evaluation metric for explanations. Finally, in the particular case of stability and correctness, we show the possible limitations of some evaluation metrics and propose new ones that take into account the local behaviour of the model under test.

==> acknowledgments.tex <==

Experiments  were carried out using the \href{https://www.grid5000.fr}{Grid'5000} testbed, supported by a scientific interest group hosted by Inria and including CNRS, RENATER and several universities and organizations.
This work has been partially supported by \grantsponsor{miai}{MIAI@Grenoble Alpes}{https://miai.univ-grenoble-alpes.fr/}, (\grantnum{miai}{ANR-19-P3IA-0003}), and \grantsponsor{tailor}{TAILOR}{https://tailor-network.eu/research-overview/} and \grantsponsor{trumpet}{TRUMPET}{https://trumpetproject.eu/}, projects funded respectively by EU H2020 research and innovation programme
    (\grantnum{tailor}{GA No 952215}) and Horizon Europe (\grantnum{trumpet}{GA No 101070038}). This work is part of the scientific network GIS Albatros (ALliance Between Universities in nouvelle Aquitaine and Thales in Research on aviOnics Systems).


==> adversarial_table.tex <==
\begin{sidewaystable}
	\centering
	\caption{Evaluating properties in an adversarial perturbation setting}\label{tab:result_adversarial} 
{\renewcommand\baselinestretch{1.1}\selectfont\resizebox{\textwidth}{!}{	\begin{tabular}{c|c|ccccccccc}
		\toprule
		\multirow{2}{*}{Property} & \multirow{2}{*}{Evaluation method} & \multicolumn{9}{c}{Saliency method}  \\
		 & & Grad-CAM  & FEM  & ML-FEM  & Grads  & Int.Grads  & SmoothGrads  & Guided Back-Prop.  & Fake-CAM  & Eye-CAM \\
		\midrule
		\multirow{3}{*}{Stability}
 		 & Stability metric ↓ & 0.070 & 1.039 & 0.215 & 0.324 & 0.373 & 0.038 & 1.187 & \textbf{0.000} & \textbf{0.000}\\
		 & Causal local explanation metric ↓ & 0.150 & 7.791 & 1.275 & \textbf{0.134} & 0.142 & 0.156 & 2.577 & 29.829 & 9.818\\
		 & Stability metric (ours) ↓ & 0.030 & 0.502 & 0.102 & 0.023 & \textbf{0.018} & 0.031 & 1.622 & 1.849 & 0.641\\
		\midrule
		\multirow{5}{*}{Correctness}
 		 & Deletion metric ↓ & 14.835/94.21 & 15.370/93.13 & 13.405/98.60 & 7.158/93.59 & 6.772/94.33 & \textbf{5.415}/95.91 & 7.442/110.42 & 19.453/7.49 & 14.490/93.89\\
		 & Average Drop ↓ & 0.176/173.71 & 0.397/204.69 & 0.220/193.71 & 0.021/111.50 & 0.022/120.19 & 0.057/109.71 & 0.030/106.61 & \textbf{0.000}/9.70 & 0.450/210.25\\
		 & Average Gain ↑ & 0.000/173.71 & 0.000/204.69 & 0.000/193.71 & \textbf{0.001}/111.50 & 0.001/120.19 & 0.000/109.71 & 0.000/106.61 & 0.000/9.70 & 0.000/210.25\\
		 & Increase in Confidence ↑ & 0.487/173.71 & 0.148/204.69 & 0.304/193.71 & \textbf{0.791}/111.50 & \textbf{0.791}/120.19 & 0.348/109.71 & 0.583/106.61 & 0.522/9.70 & 0.139/210.25\\
		 & Correctness (ours) ↓ & 0.055/17.12 & 1.617/17.12 & 0.322/17.12 & \textbf{0.036}/17.12 & 0.042/17.12 & 0.056/17.12 & 8.528/17.12 & 6.535/17.12 & 2.225/17.12\\
		\midrule
		\multirow{2}{*}{Plausibility}
 		 & Pearson Correlation Coefficient ↑ & 0.289 & 0.312 & \textbf{0.563} & 0.203 & 0.200 & 0.392 & 0.244 & 0.064 & 0.354\\
		 & Structural Similarity ↑ & 0.400 & 0.362 & 0.318 & 0.239 & 0.268 & 0.240 & 0.435 & 0.093 & \textbf{0.527}\\
	\bottomrule  
	\end{tabular}}\par} 
\end{sidewaystable}
